Learning Simplicial Complexes from Persistence Diagrams

Topological Data Analysis (TDA) studies the shape of data. A common topological descriptor is the persistence diagram, which encodes topological features in a topological space at different scales. Turner, Mukeherjee, and Boyer showed that one can reconstruct a simplicial complex embedded in R^3 using persistence diagrams generated from all possible height filtrations (an uncountably infinite number of directions). In this paper, we present an algorithm for reconstructing plane graphs K=(V,E) in R^2 , i.e., a planar graph with vertices in general position and a straight-line embedding, from a quadratic number height filtrations and their respective persistence diagrams.

==> append-constraints.tex <==
% **************** Appendix B: Algorithm for automated generation of constraints
\section{Automated Generation of Constraints}

This algorithm takes as input
\begin{itemize}
\item the locations of each vertex in an undirected graph $G = (V,E)$, and
\item the persistence diagrams of $G$ for $H_0$, $H_1$ along a single direction
$\theta_i$,
\end{itemize}
and outputs a set of graphs compatible with the diagrams.

Intuitively, each time a vertex $v$ is encountered along direction $\theta_i$,
a new set of possible undirected edges $(v,u)$ is tested for consistency with
the $H_0$, $H_1$ diagrams, where $u$ is any vertex that has already been
encountered. Here, time is the value along direction $\theta_i$ at which the
vertex is included in the filtration, possibly resulting in a birth or death.
The compatible graphs are built vertices are encountered, and partial graphs
are stored in a table $T$. Each column in $T$ corresponds to a possible edge,
and each row to a compatible graph. As vertices are added and new edges are
allowed, columns and rows are added to $T$.

%\begin{algorithm}
%\begin{algorithmic}[11]
%\Procedure{A}{$H_0$,$H_1$}
%\State ada
%\end{algorithmic}
%\end{algorithm} Impose an ordering on $V$ according to $\theta_i$ and sort the vertices from
least to greatest, resolving ambiguities arbitrarily. Let
\begin{itemize}
	\item $V'$ be the set of current vertices, and
	\item $E'$ be the set of current edges.
\end{itemize}

Initialize $V'$, $E'$ to $\emptyset$.

For $v_i \in V$ :
\begin{enumerate}
	\item for all subsets of  $v_j \in V'$
		\begin{enumerate}
			\item add column $(v_i, v_j)$ to $T$
			\item include $(v_i, v_j)$ in all the rows of $T$
			\item if row with $(v_i,v_j)$ included is incompatible
			with $H_0$ or $H_1$ do not include this
		\end{enumerate}
	\item add $v_i$ to $V'$
\end{enumerate}


==> append-transcription.tex <==
\section{Transcription of PHT Paper}
\todo{describe the edge reconstruction in terms of reconstructing a 1-complex in
$\R^2$, as a direct transcription of the Turner paper.}




==> onepoint.tex <==
%%%%% Technical details %%%%%%]
\begin{lemma}[Location of a Point]
	Let $\simComp$ be a simplicial complex composed of a single vertex
    $p\in \R^2$.
    Let $\dir_1, \dir_2 \in \sph^1$ be pairwise linearly independent.
    Let $\hFilt{\dir_1}$ and $\hFilt{\dir_2}$ be height filtrations
    from directions $\dir_1$ and $\dir_2$ respectively.
    The $(x,y)$ coordinates of $p$ can be determined using the zero-dimensional
    persistence diagrams $\dgm{0}{\dir_1}$ and $\dgm{0}{\dir_2}$ resulting from $\hFilt{\dir_1}$ and
    $\hFilt{\dir_2}$ on $\simComp$.
    \label{lem:pointLoc}
\end{lemma}
\begin{proof}
The height filtrations $\hFilt{\dir_1}$ and $\hFilt{\dir_2}$ will
encounter $p$ at a unique height.
Since $p$ is the only point in $\simComp$, $D_1$ and $D_2$ will
be composed of exactly one feature each corresponding to
the point $p$.
Then, $\pLines{\dir_1}{p}$ and $\pLines{\dir_2}{p}$ are each composed
of a single line representing the birth event of $p$ in $\dgm{0}{\dir_1}$ and
$\dgm{0}{\dir_2}$ respectively.
Since, $\dir_1$ and $\dir_2$ are linearly independent,
these lines are not parallel.
Therefore, they intersect at exactly one point.
Assume that $p$ does not lie at the point where the lines intersect.
Then, one of the
height filtrations must not have encountered $p$ at the
the height where the line corresponding to the birth lies because this line
does not intersect with $p$, a contradiction.
Therefore, the $(x,y)$ coordinates for the intersection of the two lines from
$\pLines{\dir_1}{p}$ and $\pLines{\dir_2}{p}$ are the $(x,y)$ coordinates for $p$.
\end{proof}



